Dynamical friction for supersonic motion in a homogeneous gaseous medium

The supersonic motion of gravitating objects through a gaseous medium constitutes a classical problem in theoretical astrophysics. Its application covers a broad range of objects and scales from planets up to galaxies. Especially the dynamical friction, caused by the forming wake behind the object, plays an important role for the dynamics of the system. To calculate the dynamical friction, standard formulae, based on linear theory are often used. It is our goal to check the general validity of these formulae and provide suitable expressions for the dynamical friction acting on the moving object, based on the basic physical parameters of the problem. We perform sequences of high resolution numerical studies of rigid bodies moving supersonically through a homogeneous medium, and calculate the total drag acting on the object, which is the sum of gravitational and hydro drag. We study cases without gravity with purely hydrodynamical drag, as well as gravitating objects. From the final equilibrium state of the simulations, we compute for gravitating objects the dynamical friction by direct numerical integration of the gravitational pull acting on the embedded object. The numerical experiments confirm the known scaling laws for the dependence of the dynamical friction on the basic physical parameters as derived in earlier semi-analytical studies. As a new important result we find that the shock's stand-off distance is revealed as the minimum spatial interaction scale of dynamical friction. Below this radius, the gas settles into a hydrostatic state, which causes no net gravitational pull onto the moving body. Finally, we derive an analytic estimate for the stand-off distance that can be used to calculate the dynamical friction force.

==> makefile <==
LATEX = pdflatex
FLAGS = -interaction=nonstopmode

BIBTEX = bibtex

RM =rm -rf

MAIN = df
BIB_FILE = Papers_DT.bib Papers_RK.bib

TEX := $(shell find . -name '*.tex' -print)
PDF := $(shell find plots/ -name '*.pdf' -print)
PNG := $(shell find plots/ -name '*.png' -print)
OBJ = $(MAIN).aux $(MAIN).bbl

all: $(MAIN).pdf

$(MAIN).pdf: $(TEX) $(PDF) $(PNG) $(OBJ) makefile
	@echo "--- Running $(LATEX) $(MAIN).tex ---"
	$(LATEX) $(FLAGS) $(MAIN).tex | tee $(MAIN).$(LATEX)_output
	@while ( grep -q 'Rerun to get' $(MAIN).log ) ; do                    \
			echo "--- Rerunning $(LATEX) $(MAIN).tex ---" ;               \
			$(LATEX) $(FLAGS) $(MAIN).tex | tee $(MAIN).$(LATEX)_output ; \
	done

$(MAIN).aux: $(TEX)
	@echo "--- Running $(LATEX) $(MAIN).tex to get $(MAIN).aux-file ---"
	$(LATEX) $(MAIN).tex

$(MAIN).bbl: $(BIB_FILE)
	@echo "--- Running $(BIBTEX) $(MAIN).tex to get $(MAIN).bbl-file ---"
	$(BIBTEX) $(MAIN)

clean:
	$(RM) $(MAIN).aux $(MAIN).bbl $(MAIN).blg $(MAIN).log $(MAIN).out \
		  $(MAIN).toc $(MAIN).$(LATEX)_output $(MAIN).llt

